Generalizing Monocular 3D Object Detection

Monocular 3D object detection (Mono3D) is a fundamental computer vision task that estimates an object's class, 3D position, dimensions, and orientation from a single image. Its applications, including autonomous driving, augmented reality, and robotics, critically rely on accurate 3D environmental understanding. This thesis addresses the challenge of generalizing Mono3D models to diverse scenarios, including occlusions, datasets, object sizes, and camera parameters. To enhance occlusion robustness, we propose a mathematically differentiable NMS (GrooMeD-NMS). To improve generalization to new datasets, we explore depth equivariant (DEVIANT) backbones. We address the issue of large object detection, demonstrating that it's not solely a data imbalance or receptive field problem but also a noise sensitivity issue. To mitigate this, we introduce a segmentation-based approach in bird's-eye view with dice loss (SeaBird). Finally, we mathematically analyze the extrapolation of Mono3D models to unseen camera heights and improve Mono3D generalization in such out-of-distribution settings.

==> images/deviant/teaser_common.tex <==
\node[inner sep=0pt] (input) at (7.5,10.0) {\includegraphics[height=3.0cm]{images/deviant/pink_car_back.png}};
    
%===== Image on the image plane  ======
\draw [draw=projectionBorderShade, line width=0.02em, fill=projectionFillShade]    (2.2, 3.2) rectangle (6.8, 6.2) node[]{};
\node[inner sep=0pt] (input) at (3.6,4.8) {\includegraphics[height=1.5cm]{images/deviant/pink_car_back.png}};

\draw [draw=projectionBorderShade, line width=0.02em, fill=projectionFillShade]    (-2.0, -2.6) rectangle (2.6, 0.2) node[]{};
\node[inner sep=0pt] (input) at (-0.75,-1.0) {\includegraphics[height=0.8cm]{images/deviant/pink_car_back.png}};
 

 
%============ Left Shooting rays (Bottom two) ================= 
\draw [draw=rayShade, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (3.6,4.8) node[]{}
    -- (0.15,0.2) node[]{};
    
\draw [draw=rayShade, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (-0.75,-1.0) node[]{}
    -- (-3.0,-4.0) node[]{};    


%============ Movement ================= 
\draw [-{Triangle[angle=60:.1cm 1]}, draw=proposedShade, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (-0.25,3.0) node[]{}
    -- (-5.01,-2.68) node[pos=0.5, scale= 2.5, align= center]{\color{proposedShade}{$\transZ$}~~~~\\};
    

%================ Cameras =========================
% Camera left top
\draw[black, fill=black!50, densely dashed, line width=0.05em, rotate around={53:(1.5,2.0)}] (0.9,1.6) rectangle (2.1,2.4);
% coordinates
\coordinate (c00) at (1.86,2.48);
\coordinate (c01) at (1.86,3.00);
\coordinate (c02) at (2.4,2.6);
\filldraw[draw=black, fill=gray!20, densely dashed, line width=0.05em] (c00) -- (c01) -- (c02) -- cycle;

% Camera left bottom
\draw[black,fill=black!50,rotate around={53:(-3,-4.0)}] (-3.6,-4.4) rectangle (-2.4,-3.6);
\coordinate (c10) at (-2.64,-3.52);
\coordinate (c11) at (-2.64,-3.0);
\coordinate (c12) at (-2.1,-3.4);
\filldraw[draw=black, fill=gray!20] (c10) -- (c11) -- (c12) -- cycle;

==> images/groomed/block_diagram_common.tex <==
    % trim={<left> <lower> <right> <upper>}
    %\node[inner sep=0pt] (input) at (-3,0) {\includegraphics[trim={20.3cm 0 12.5cm 5.4cm},clip,height=2cm]{images/000952.png}};
    %\node[inner sep=0pt] (input) at (-2.1,0) {\includegraphics[trim={19.1cm 1.8cm 18.7cm 5.6cm},clip,height=2cm]{images/007416.png}};
    \node[inner sep=0pt] (input) at (1.2,0) {\includegraphics[trim={20.9cm 4.2cm 18.75cm 5.6cm},clip,height=1.1cm]{images/groomed/007396.png}};
    
    %===== Backbone ======
    \draw [draw=black, fill= my_yellow!40, line width=0.06em, thick] 
       (2.5, 3.0) node[]{}
    -- (2.5,-3.0) node[pos= 0.8, right, scale= 1.25, rotate=90, align=center]{~\\~\\Backbone}
    -- (4,-2.0) node[]{}
    -- (4, 2.0) node[]{}
    -- cycle;
    
    %======== Heads ========
    \draw [draw=black, fill= my_blue!40, line width=0.06em, thick] (5, 1.8) rectangle (7.5,0.8) node[pos=0.5, scale= 1.25]{Score};
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=my_blue!50, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (4.0,1.2) node[]{}
    -- (5.0,1.2) node[]{};

    \draw [draw=black, fill= blue!20, line width=0.06em, thick] (5, 0.5) rectangle (7.5, -0.5) node[pos=0.5, scale= 1.25]{$\twoD$};
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=blue!30, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (4.0,0) node[]{}
    -- (5.0,0) node[]{};
    
    \draw [draw=black, fill= my_violet!20, line width=0.06em, thick] (5, -0.8) rectangle (7.5, -1.8) node[pos=0.5, scale= 1.25]{$\threeD$};
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=my_violet!40, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (4.0,-1.3) node[]{}
    -- (5.0,-1.3) node[]{};

    %============== Towards NMS ==============
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=my_blue!50, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (7.5,1.2) node[]{}
    -- (12.25,1.2) node[pos=0.84, scale= 1.25, align=center]{$\score$\\};
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=blue!30, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (7.5,0) node[]{}
    -- (12.25 ,0) node[pos=0.84, scale= 1.25, align=center]{$\overlapMat$\\};
    \draw [, draw=my_violet!40, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (7.5,-1.2) node[]{}
    -- (8.1,-1.2) node[]{};

    %============== Towards Loss ==============
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=my_blue!50, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (9.0,1.2) node[]{}
    -- (9.0,-2.8) node[]{};
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=blue!30, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (8.5,0) node[]{}
    -- (8.5,-2.7) node[]{};
    \draw [-{Triangle[angle=60:.1cm 1]}, draw=my_violet!40, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (8, -1.2) node[]{}
    -- (8,-2.8) node[]{};
    
    %================ Circles/Connector ===============
    \draw[draw=my_blue!50, fill=my_blue!50, thick](9,1.2) circle (0.15) node[scale= 1.25]{};
    \draw[draw=blue!30, fill=blue!30, thick](8.5,0) circle (0.15) node[scale= 1.25]{};

    %======== IOU ========
    \draw [draw=black, fill= my_orange!80, line width=0.06em] (9.5,0.5) rectangle (11,-0.5) node[pos=0.5, scale= 1.25]{\iou};
    
    %============ Loss Before=============
    \draw[draw=black, fill=my_red!30, thick]( 8.5,-4.2) circle (1.5) node[scale= 1.25]{$\lossBefore$};
    
    %============ Box Proposals before NMS ================
    \draw [draw=green!80, line width=0.06em]                (5.6, 3.2) rectangle (8.15, 4.85) node[]{};
    \draw [draw=cyan, line width=0.06em]                    (5.4, 2.8) rectangle (7.9   , 5 ) node[]{};
    \draw [draw=orange!80, line width=0.06em, thick]        (5.2, 3.0) rectangle (7.7 , 5.25) node[]{};
    \draw [draw=red, line width=0.06em, very thick]         (5  , 3.5) rectangle (7.5 , 5.5   ) node[]{};

    \draw [draw=purple!80, line width=0.06em, thick]        (8.7, 3.0) rectangle (9.20, 5  ) node[]{};
    \draw [draw=my_yellow_2, line width=0.06em, very thick] (8.5, 3.5) rectangle (9   , 5.25) node[]{};

    
    \node [inner sep=1pt, scale= 1.25] at (6.8, 2.35)  {$\boxes$};
    
    %=========== Training inference arrows===========
    \draw [-{Triangle[angle=60:.1cm 1]}, dashed, draw=black!40, line width=0.1em, shorten <=0.5pt, shorten >=0.5pt, >=stealth]
       (0.5,7) node[]{}
    -- (20,7) node[pos= 0.9, align=center, scale= 1.25]{Inference\\};
